Revisiting Transactional Statistics of High-scalability Blockchains

Scalability has been a bottleneck for major blockchains such as Bitcoin and Ethereum. Despite the significantly improved scalability claimed by several high--profile blockchain projects, there has been little effort to understand how their transactional throughput is being used. In this paper, we examine recent network traffic of three major high-scalability blockchains--EOSIO, Tezos and XRP Ledger (XRPL)--over a period of seven months. Our analysis reveals that only a small fraction of the transactions are used for value transfer purposes. In particular, 96% of the transactions on EOSIO were triggered by the airdrop of a currently valueless token; on Tezos, 76% of throughput was used for maintaining consensus; and over 94% of transactions on XRPL carried no economic value. We also identify a persisting airdrop on EOSIO as a DoS attack and detect a two-month-long spam attack on XRPL. The paper explores the different designs of the three blockchains and sheds light on how they could shape user behavior.

==> sections/b_extra.tex <==
\section{Additional Tables and Figures}
\label{sec:extra}
In this section, we include table and figures which are relevant to the paper but were not important enough to be included in the main content.
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{figures/tweetxrp}
%     \caption{A tweet questioning the transaction value on XRPL \cite{LordofCrypto2018}.
%     }
%     \label{fig:tweetxrp}
% \end{figure}




% \input{sections/tables/eos-top-senders}






==> sections/tables/eos-top-senders.tex <==

\begin{figure*}
    \footnotesize
    \centering
    \begin{tabular}{l r r l r r}
    \toprule
    \bf Sender & \bf Sent count & \bf Unique & \bf Receiver & \# \bf of transactions & \% \bf of transactions\\
    &  & \bf receivers & & &\\
    \midrule
    \multirow{5}{*}{betdicegroup} &  \multirow{5}{*}{35,150,255} & \multirow{5}{*}{34} & betdicetasks & 24,244,530 & 68.90\%\\
    & & & {betdicegroup} & 4,768,591 & 13.55\%\\
    & & & betdicebacca & 1,812,993 & 5.15\%\\
    & & & betdicesicbo & 1,770,341 & 5.03\%\\
    & & & betdiceadmin & 1,224,500 & 3.48\%\\
    \midrule
    \multirow{2}{*}{mykeypostman} & \multirow{2}{*}{11,778,190} & \multirow{2}{*}{7} & eosio.token & 138,639,137 & 94.04\%\\
    & & & mykeylogica1 & 8,689,661 & 5.89\%\\
    \midrule
    \multirow{5}{*}{bluebetproxy} & \multirow{5}{*}{6,255,614} & \multirow{5}{*}{16} & bluebetproxy & 3,136,527 & 50.14\%\\
    & & & eosio.token & 1,817,302 & 29.05\%\\
    & & & bluebettexas & 522,041 & 8.35\%\\
    & & & bluebetjacks & 182,511 & 2.92\%\\
    & & & bluebetbcrat & 177,748 & 2.84\%\\
    \midrule
    \multirow{2}{*}{bluebet2user} & \multirow{2}{*}{5,781,071} & \multirow{2}{*}{15} & lynxtoken123 & 5,574,173 & 96.42\%\\
    & & & eosio.token & 51,723 & 0.89\%\\
    \midrule
    \multirow{2}{*}{bluebetbcrat} & \multirow{2}{*}{5,490,267} & \multirow{2}{*}{15} & bluebetbcrat & 4,346,721 & 79.17\%\\
    & & & eosio.token & 1,016,165 & 18.51\%\\
    \bottomrule
    \end{tabular}
    \caption{EOSIO account pairs with the highest number of sent transactions.}
    \label{tab:eos-account-edges}
\end{figure*}
